Fast Algorithms for $\ell_p$-Regression

The $\ell_p$-norm regression problem is a classic problem in optimization with wide ranging applications in machine learning and theoretical computer science. The goal is to compute $x^{\star} =\arg\min_{Ax=b}\|x\|_p^p$, where $x^{\star}\in \mathbb{R}^n, A\in \mathbb{R}^{d\times n},b \in \mathbb{R}^d$ and $d\leq n$. Efficient high-accuracy algorithms for the problem have been challenging both in theory and practice and the state of the art algorithms require $poly(p)\cdot n^{\frac{1}{2}-\frac{1}{p}}$ linear system solves for $p\geq 2$. In this paper, we provide new algorithms for $\ell_p$-regression (and a more general formulation of the problem) that obtain a high-accuracy solution in $O(p n^{\frac{(p-2)}{(3p-2)}})$ linear system solves. We further propose a new inverse maintenance procedure that speeds-up our algorithm to $\widetilde{O}(n^{\omega})$ total runtime, where $O(n^{\omega})$ denotes the running time for multiplying $n \times n$ matrices. Additionally, we give the first Iteratively Reweighted Least Squares (IRLS) algorithm that is guaranteed to converge to an optimum in a few iterations. Our IRLS algorithm has shown exceptional practical performance, beating the currently available implementations in MATLAB/CVX by 10-50x.

==> Chapters/Sparsification.tex <==
%!TEX root = ../mainJournal.tex

\section{Almost-Linear-Time Weighted \texorpdfstring{$\ell_p$}{TEXT}-norm Solvers in Slightly Dense Graphs via Sparsification}

In this section we show how we can use our algorithms to obtain high accuracy solutions for $\ell_p$-regression for $\ell_p$-norm flow and voltage problems on graphs which we will define shortly. We will further give faster algorithms for these problems by using the sparsification techniques from \cite{AdilBKS21}.

\subsection{Flow and Voltage Problems}
A network flow problem on a graph $G$ with $n$ vertices and $m$ edges is defined as,
\[
\min_{\BB^{\top}\ff = \dd} \text{cost}(\ff),
\]
where $\ff \in \mathbb{R}^m$ is a vector defining flows on the edges of the graph, $\BB$ is the edge-vertex incidence matrix of the graph and $\dd$ is a vector defining net demands on every vertex. This general formulation captures some widely studied problems, such as, cost$(\ff) = \|\SS^{-1}\ff\|_{\infty}$ captures the maximum flow problem with capacities $\SS$; cost$(\ff)= \|\SS\ff\|_1$ captures the transshipment problem; and cost$(\ff) = \ff^{\top}\RR\ff$ captures the electrical flow problem. We can similarly define voltage problems which are dual to flow problems as,
\[
\min_{\dd^{\top}\vvs} \text{cost}'(\BB\vvs).
\]  
The voltage problem also captures a few widely studied problems, such as, $\text{cost}'(\BB\vvs) = \|\SS\BB\vvs\|_1$ captures the min-cut problem; $\text{cost}'(\BB\vvs) = \|\SS\BB\vvs\|_{\infty}$ captures vertex-labeling \cite{KyngRSS15}; and $\text{cost}'(\BB\vvs) = \|\RR^{-\frac{1}{2}}\BB\vvs\|_2^2$  captures the electrical voltages problem. In this section we will focus on the $\ell_p$-norm, $p\geq 2$, flow and voltage problems which are defined as follows.

\begin{definition}\label{def:flow}{($\ell_p$ Flow Problem).} Given a graph $G(V,E)$ with non-negative diagonal matrices $\RR,\SS \in \mathbb{R}^{E\times E}$, and a gradient vector $\gg \in \mathbb{\RR}^E$, we define the $\ell_p$-norm flow problem as,
\[
\min_{\BB^{\top}\ff = \dd} \gg^{\top}\ff + \|\RR^{1/2}\ff\|_2^2 + \|\SS\ff\|_p^p.
\]
We also have, $\gg \perp \{ker(\RR)\cap ker(\SS) \cap ker(\BB)\}$, so that the problem has a bounded solution and  $\dd \perp 1$ so that a solution exists.
\end{definition}

\begin{definition}\label{def:voltage}{($\ell_p$ Voltage Problem).} Given a graph $G(V,E)$ with non-negative diagonal matrices $\WW,\UU \in \mathbb{R}^{E\times E}$, and demands $\dd \in \mathbb{\RR}^V$ with $\dd\perp 1 = 0$, we define the $\ell_p$-norm voltage problem as,
\[
\min_{\vvs} \dd^{\top}\vvs + \|\WW^{1/2}\BB\vvs\|_2^2 + \|\UU\vvs\|_p^p.
\]
\end{definition}

\subsection{Results and Related Works}
The following is directly from \cite{AdilBKS21}

\paragraph{Progress on Dense Graphs}
We obtain a nearly-linear running time for $\ell_p$ flow/voltage problems on graphs. Our algorithm requires 
$p(m^{1+o(1)} + n^{4/3 + o(1)})$ time for $p=\omega(1)$ which is almost-linear-time for $p \leq m^{o(1)}$ in slightly dense graphs, ($m \ge n^{4/3 + o(1)}$).

Recently, there has been progress on dense graph problems. In \cite{van2020bipartite}, the authors developed an algorithm for weighted bipartite matching and transshipment running in $\Otil(m + n^{3/2})$ time. Our running time $m^{1+o(1)} + n^{4/3+o(1)}$ is even better than the runtime of \cite{van2020bipartite}. Our result beats the $\Omega(n^{3/2})$ barrier that arises from the use of interior point methods that maintain a vertex  dual solution using dense updates across $\sqrt{n}$ iterations. The progress on bipartite matching relies on highly technical graph-based inverse maintenance techniques that are tightly interwoven with interior point
method analysis. In constrast, our sparsification methods provide a clean interface to iterative refinement, which makes our analysis much more simple and compact.


\paragraph{Graph Sparsification}
Various notions of graph sparsification -- replacing a dense graph with a sparse one, while approximately preserving some key properties of the dense graph  -- have been key ingredients in faster low-accuracy algorithms. Bencz\'{u}r and Karger~\cite{BenczurK96} defined cut-sparsifiers that approximately preserve all cuts, and used them to give faster low-accuracy approximation algorithms for maximum-flow. Since then, several notions of sparsification have been studied extensively and
utilized for designing faster algorithms~\cite{PelegS89, SpielmanT11, Racke08, SpielmanS11, Madry10, Sherman13, KelnerLOS14, RackeST14, CohenP15, KyngLPSS16, DurfeePPR17, ChuGPSSW18}.
%

Sparsification has had a smaller direct impact on the design of faster high-accuracy algorithms for graph problems, limited mostly to the design of linear system solvers~ \cite{SpielmanT04, KoutisMP11, PengS14, KyngLPSS16}. Kyng~\etal~\cite{kyngPSW19} constructed sparsifiers for weighted $\ell_2^{2}$ + unweighted $\ell_{p}^{p}$-norm objectives for flows. In \cite{AdilBKS21}, we develop almost-linear time algorithms for building sparsifiers for weighted $\ell_2^{2} + \ell_{p}^{p}$ norm objectives
for flows and voltages,
\[
  cost(\ff) = \|\RR^{\frac{1}{2}} \ff \|_2^{2} + \|\SS \ff \|_p^{p}
  ,\text{ and } cost'(\BB\vvs) = \|\WW^{\frac{1}{2}} \BB \vvs \|_2^{2} + \|\UU \BB \vvs \|_p^{p},
\]
and utilize them as key ingredients in our faster high-accuracy algorithms for optimizing such objectives on graphs. Our construction of sparsifiers for flow objectives builds on the machinery from~\cite{kyngPSW19}, and our construction of sparsifiers for voltage objectives builds on graph spanners~\cite{AlthoferDDJS93,
  PelegS89, BaswanaS07}.

\subsubsection{Fast, High-Accuracy Algorithms}

Observe that these problems directly fit into our general framework for $\ell_p$-norm regression. We can thus directly apply algorithms from previous sections to obtain high-accuracy algorithms. Specifically, we can use Algorithm \ref{alg:CompleteLp} directly for these problems. From Theorem \ref{thm:CompleteLp}, the rates of convergence for these problems are thus $\Otil(pm^{1/3})$ calls to a linear system solver. Further observe that the linear systems being solved for these graph instances are laplacian linear systems, and using fast solvers we can solve these in near linear time \cite{spielman2014nearly}. Therefore, the total runtime of our algorithm when applied directly is $\Otil(pm^{4/3})$. We will now utilize sparsification routines from \cite{AdilBKS21} and combine these with our algorithm to obtain a runtime of $p\left(m^{1+o(1)} + n^{4/3 + o(1)}\right)$.

\subsubsection{Sparsification Results for Flow and Voltage Problems}
The following are the sparsification results from \cite{AdilBKS21}.

\begin{theorem}\label{thm:flowSparse}
(Theorem 2.3 \cite{AdilBKS21}) Consider a graph $G$ with $n$ vertices and $m$ edges, equipped with non-negative $\ell_2$ and $\ell_p$-weights, as well as a gradient. In $\Otil(m)$ time, we can compute a graph $H$ with $n$ vertices and $\Otil(n)$ edges, equipped with non-negative $\ell_2$ and $\ell_p$-weights, as well as a gradient, such that a constant factor approximation to the flow residual problem on $H$, when scaled by $m^{-\frac{1}{p-1}}$ results in an $\Otil\left(m^{\frac{2}{p-1}}\right)$ approximate solution to the flow residual problem on $G$. The algorithm works for all $p \geq 2$ and succeeds with high probability.
\end{theorem}

\begin{theorem}\label{thm:voltageSparse}
(Theorem 2.4 \cite{AdilBKS21}) Consider a graph $G$ with $n$ vertices and $m$ edges, equipped with non-negative $\ell_2$ and $\ell_p$-conductances. In $\Otil(m)$ time, we can compute a graph $H$ with $n$ vertices and $\Otil(n)$ edges, equipped with non-negative $\ell_2$ and $\ell_p$-conductances, such that a constant factor approximation to the flow residual problem on $H$, when scaled by $m^{-\frac{1}{p-1}}$ results in an $\Otil\left(m^{\frac{1}{p-1}}\right)$ approximate solution to the flow residual problem on $G$. The algorithm works for all $p \geq 2$ and succeeds with high probability.
\end{theorem}

We can utilize the above sparsification routines to compute smaller sized instances of the residual problems quickly, and apply our residual problem solvers on these smaller instances. This procedure is described in Algorithm \ref{alg:SparseLp}.

\begin{algorithm}[H]
\caption{Algorithm for $\ell_p$ Flows and Voltages}
\label{alg:SparseLp}
 \begin{algorithmic}[1]
 \Procedure{\textsc{$\ell_p$-Solver}}{$\AA, \MM,\NN, \dd,\bb,p,\epsilon$}
\State $\xx \leftarrow \xx^{(0)}$
\State $\nu \leftarrow \ff(\xx^{(0)})$
\State $\widetilde{\kappa} \leftarrow \begin{cases}
m^{\frac{2}{p-1}}, & \text{ if flow problem}\\
m^{\frac{1}{p-1}}, & \text{ if voltage problem}
\end{cases}$
\While{$\nu >\frac{\epsilon}{2} \ff(\xx)$}
\State $(\widetilde{\gg},\widetilde{\RR},\widetilde{\NN}) \leftarrow$ Sparsify$(\gg,\RR,\NN)$\Comment{$\gg,\RR,\NN$ are from the residual problem}
\If{$p \geq \log m$}
\State $\Dtil \leftarrow$ $\log m$-ResidualSolver
\Else 
\State $\Dtil \leftarrow$ ResidualSolver
\EndIf
\If{$\res_p(m^{-\frac{1}{p-1}}\Dtil) \geq \frac{\nu}{32p\kappa \widetilde{\kappa}}$}
\State $\xx \leftarrow \xx - \frac{\Dtil}{p}$ 
\Else
\State $\nu \leftarrow \frac{\nu}{2}$
\EndIf
\EndWhile
\State \Return $\xx$
 \EndProcedure 
 \end{algorithmic}
\end{algorithm}
Algorithm \ref{alg:SparseLp} has the following guarantees which follows directly from the application of Theorems \ref{thm:flowSparse}, \ref{thm:voltageSparse} with Theorem \ref{thm:CompleteLp}, and using fast near linear time laplacian solvers to solve linear systems. These theorems are similar to Theorems 2.1 and 2.2 in \cite{AdilBKS21}.

\begin{theorem}(Flow Algorithmic Result.) Consider a graph $G$ with $n$ vertices and $m$ edges, equipped with non-negative $\ell_2$ and $\ell_p$-weights, as well as a gradient and demands. For $p = \omega(1)$, in $p\left(m^{1+o(1)}+n^{4/3+o(1)}\right)\log\frac{1}{\epsilon}$ time we can compute an $\epsilon$-approximately optimal flow to Problem \ref{def:flow} with high probability.
\end{theorem}

\begin{theorem}(Voltage Algorithmic Result.) Consider a graph $G$ with $n$ vertices and $m$ edges, equipped with non-negative $\ell_2$ and $\ell_p$-conductances, as well as demands. For $p = \omega(1)$, in $p\left(m^{1+o(1)}+n^{4/3+o(1)}\right)\log\frac{1}{\epsilon}$ time we can compute an $\epsilon$-approximately optimal flow to Problem \ref{def:voltage} with high probability.
\end{theorem}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "thesis"
%%% End:

